Learning Discriminative Model Prediction for Tracking

The current strive towards end-to-end trainable computer vision systems imposes major challenges for the task of visual tracking. In contrast to most other vision problems, tracking requires the learning of a robust target-specific appearance model online, during the inference stage. To be end-to-end trainable, the online learning of the target model thus needs to be embedded in the tracking architecture itself. Due to the imposed challenges, the popular Siamese paradigm simply predicts a target feature template, while ignoring the background appearance information during inference. Consequently, the predicted model possesses limited target-background discriminability. We develop an end-to-end tracking architecture, capable of fully exploiting both target and background appearance information for target model prediction. Our architecture is derived from a discriminative learning loss by designing a dedicated optimization process that is capable of predicting a powerful model in only a few iterations. Furthermore, our approach is able to learn key aspects of the discriminative loss itself. The proposed tracker sets a new state-of-the-art on 6 tracking benchmarks, achieving an EAO score of 0.440 on VOT2018, while running at over 40 FPS. The code and models are available at https://github.com/visionml/pytracking.

==> tables/ablation_loss.tex <==
\begin{tabular}{l@{~}c@{~~}}
\toprule
&TD323\\\midrule
L2 train L2 test&n\\
hinge train hinge test&n\\
learned train hinge test&\\\bottomrule

\end{tabular}


==> tables/lasot.tex <==
\begin{tabular}{l@{~}c@{~~}c@{~~}c@{~~}c@{~~}c@{~~}c@{~~}c@{~~}c@{~~}c@{~~}c@{~~}c@{~~}}
	\toprule
	&ECO&DSiam&StructSiam&SiamFC&VITAL&MDNet&DaSiamRPN&SiamRPN++&ATOM&ETCOM18&ETCOM50\\\midrule
	Norm.\ Prec. (\%)&33.8&40.5&41.8&42.0&45.3&46.0&49.6&56.9&57.6&\textbf{\textcolor{blue}{61.5}}&\textbf{\textcolor{red}{64.6}}\\
	Success (\%)&32.4&33.3&33.5&33.6&39.0&39.7&41.5&49.6&51.5&\textbf{\textcolor{blue}{53.5}}&\textbf{\textcolor{red}{56.6}}\\\bottomrule
\end{tabular}


==> tables/vot_less_data.tex <==
\begin{tabular}{lcc}
	\toprule
	&SiamRPN++&DiMP-50-data\\\midrule
	EAO&0.414&0.416\\
	Robustness&0.234&0.181\\
	Accuracy&0.600&0.593\\\bottomrule
\end{tabular}

